On the classification of laminations associated to quadratic polynomials

Given any rational map $f$, there is a lamination by Riemann surfaces associated to $f$. Such laminations were constructed in general by Lyubich and Minsky. In this paper, we classify laminations associated to quadratic polynomials with periodic critical point. In particular, we prove that the topology of such laminations determines the combinatorics of the parameter. We also describe the topology of laminations associated to other types of quadratic polynomials.

==> topologyb.tex <==
\section{Topology of inverse limits}

\subsection{The laminated Julia set}

Let $\mc{J}_c=\pi^{-1}(J_c)\cap \mc{R}_c$ be the lift of the Julia
set on the regular part. We call $\mc{J}_c$ the \textit{laminated
Julia set} associated to $f_c$. If $c$ is a convex co-compact
parameter, by a theorem in \cite{LM}, $\mc{J}_c$ is compact inside
$\mc{R}_c$ with the natural topology. When $c$ is convex
cocompact, there are no irregular points on the laminated Julia
set $\mc{J}_c$.

In this section we discuss the topological properties of
$\mc{J}_c$. Given a repelling periodic point $q$ in the dynamical
plane, let us denote by $\h{q}$ the periodic point in the regular
part which satisfies $\pi(\h{q})=q$. Let $\mathcal{P}$ be the set
of repelling periodic points in $\mc{R}_{c}$.


\subsubsection{Leafwise connectivity of $\mc{J}_c$}

\begin{lemma}\label{lcdisconnection}
Let $c$ be a parameter with locally connected Julia set,
$\overline{P(f_c)}\neq J_c$, and such that $\pi^{-1}(J(f_c))$
contains an irregular point in the natural extension $\mc{N}_c$.
Then, there is a leaf $L$ in the regular part $\mc{R}_{c}$, such
that $\mc{J}_c \cap L$ is disconnected.
\end{lemma}

\begin{proof} Let $\hat{z}$ be an irregular point in the Julia set in
$\mc{N}_c$ then, since $J(f_c)$ is completely invariant and
locally connected, $\pi_{-j}(\hat{z})=z_{-j}$ belongs to $J(f_c)$
and there is an external ray $R(j)$ landing at $z_{-j}$ for every
$j$. Let $r_0$ be a point in $R(0) \cap A(\infty)$, by pulling
back $r_0$ along the backward orbit determined by $\hat{z}$, there
is a point $\h{r} \in \mc{R}_c$ such that $\pi(\h{r})=r_0$ and
$\pi_{-j}(\h{r})\subset R(j)$, now by moving $r_0$ along the ray
$R(0)$, we construct a line $\h{R}$ in the regular part, such that
$\pi_{-j}(\h{R})=R(j)$. Let $L$ be the leaf in the regular part
containing $\h{R}$. By construction the endpoints of $\h{R}$ are
the irregular points $\h{z}$ and $\h{\infty}$, this line can not
have accumulation points in $\mc{R}_c$ when $r_0$ either tends to
$z_0$ or to $\infty$. So, $\h{R}$ is a line escaping to infinity
in both directions and separates $L$ in two pieces.

Now, fix $r_0$ in the external ray $R(0)$, let $a\in J(f_c)
\setminus\overline{P(f_c)}$, and choose two paths, $\sigma_1$ and
$\sigma_2$, from $r_0$ to $a$ starting at different directions
with respect to the ray $R(0)$, and such that none of them crosses
$R(0)$ again. These two paths lifts to paths in $L$, joining
$\h{r}$ with points in $\mc{J}_c\cap L$, by construction the
points lie on different sides of the line $\h{R}$. Therefore
$\mc{J}_c\cap L$ is disconnected.
\end{proof}


As interesting examples we can point: quadratic polynomials with
parabolic cycles (see Tomoki Kawahira's paper \cite{Tom}), or the
Feigenbaum quadratic polynomial. In the case of quadratic
polynomials with parabolic cycles, leaves in the regular part
where the Julia set is disconnected are precisely the periodic
leaves corresponding to the parabolic cycle. As for repelling
cycles the linearizing coordinate, in this case Fatou's
coordinate, gives a uniformization of the periodic leaves on the
regular part. A detail explanation and construction of such
uniformization can be found in \cite{Tom}. Is worth noting that,
when $f_c$ is parabolic, then for any leave $L$ the set
$\mc{J}_c\cap L$ consists of finitely many components.



In general, it is not clear whether the intersection of the
laminated Julia set consists of finitely many pieces. An
interesting example to bear in mind is the natural extension
associated to the Feigenbaum polynomial. In this case, there are
irregular points in the fiber of the Julia set, and then there are
leaves for which the Julia set is not path connected.

As a corollary, if under the conditions of Lemma
\ref{lcdisconnection} the laminated Julia set $\mc{J}_c$ is
leaf-wise connected, then there are no irregular points in
$\mc{J}_c$, which implies that $f_c$ is convex co-compact. The
following Lemma shows that the converse is also true:

\begin{lemma}\label{leafwise.con} If $c$ is a convex cocompact
parameter, then the set $\mc{J}_c$ is leafwise connected.
\end{lemma}

\begin{proof} Since $f_c$ is convex cocompact, then the Julia set
$J(f_c)$ is locally connected and every external ray lands in the
Julia set. Moreover, since there is no irregular point on
$\pi^{-1}(J(f_c)$ in $\mc{N}_{f_c}$, every solenoidal ray also
lands at $\mc{J}_c$. Let $L$ be a leaf in the regular part, and
let $\h{z}$ and $\h{\zeta}$ be two points in $L\cap \mc{J}_c$.
Since $\h{z}$ and $\h{\zeta}$ belong to the same leaf, there exist
a path $\sigma$ in $L$ joining $\h{z}$ with $\h{\zeta}$. Then by
using the external ray flow in $L$ the path $\sigma$ projects onto
a path whose trajectory lies in $\mc{J}_c$ and connects $\h{z}$
with $\h{\zeta}$, so $\h{z}$ and $\h{\zeta}$ lie in the same
connected component of $L\cap \mc{J}_c$.
\end{proof}

Together, Lemma~\ref{lcdisconnection} and Lemma~\ref{leafwise.con}
imply:

\begin{proposition}
A quadratic parameter $c$ with locally connected Julia set
$J(f_c)$ and $\overline{P(f_c)}\neq J_c$ has leafwise connected
Julia set $\mc{J}_c$ in its regular part $\mc{R}_c$, if and only
if $c$ is convex cocompact.
\end{proposition}

\subsection{Unbounded Fatou components}

Let $\mc{F}_c=\pi^{-1}(F(f_c))\cap\mc{R}_{c}$ be the lift of the
Fatou set to the regular part. Given an affine leaf $L$ in
$\mc{R}_{c}$, consider the uniformization $\phi:L\rightarrow \C$.
We call a subset $A$ in $L$ \textit{bounded}, if the corresponding
set $\phi(A)$ is bounded in $\mathbb{C}$.

\begin{lemma} Let $f_c$ be a convex cocompact quadratic polynomial,
and let $A$ be a Fatou component of $\mc{F}_c$ inside an affine
leaf $L$. Then $A$ is bounded if and only if the restriction
$\pi|_A$ has finite degree.
\end{lemma}

\begin{proof} If the dynamical Fatou set consist only of the basin
of infinity, then all Fatou components in $\mc{F}_c$ are
unbounded, this is because the lift of B\"ottcher's coordinate
maps $\pi^{-1}(A(\infty))$ to an open solenoidal cone, and each
leaf of this cone has $\h{\infty}$ on the boundary. Moreover,
since the fiber of any point on the solenoidal cone at infinity
intersects each leaf infinitely many times, the restriction of
$\pi|A$ over every leaf of the solenoidal cone has infinite
degree.

The remaining case is when $f_c$ is hyperbolic. By the same
argument above, every Fatou component $A$ in $\pi^{-1}(A(\infty))$
is unbounded and the restriction $\pi|_A$ has infinite degree. So
let $A$ a Fatou component in $\mc{F}_c$ such that $\pi(A)$ is
bounded in the dynamical plane. Since $f_c$ is hyperbolic,
$\pi(A)$ is actually simply connected and the boundary
$\partial(\pi(A))$ is a Jordan closed curve. The set $A$ is
bounded if and only if $\partial(A)$ is bounded. The lift of
$\partial(\pi(A))$ is also a Jordan curve, say $C$, so $C$ bounded
if and only if $\pi|_C$ has finite degree, but $\pi|_C$
corresponds to the degree of $\pi|_A$.
\end{proof}

We want to count how many unbounded Fatou components there are in
$L$.


\begin{proposition}\label{unbounded} Let $f_c$ be a quadratic
polynomial and let $L$ be a periodic affine leaf in the regular
part $\mc{R}_{f_c}$ containing a periodic point $\h{p}$. Then, the
number of unbounded Fatou components of $L\setminus \mc{J}_c$ is
either $2v_p$, if the corresponding periodic point $p$ belongs to
the dynamic root cycle and $c$ belongs to a satellite hyperbolic
component; $3$ if $p$ belongs to the dynamic root cycle and $c$ is
in a primitive hyperbolic component, finally is $v_p$ otherwise.
\end{proposition}

\begin{proof} Since Siegel periodic points lift into hyperbolic leaves in
$\mc{R}_c$, by Lemma~\ref{lamin.julia}, $p$ most be a repelling
periodic point. In the dynamical plane, there are $v_p$ rays
landing at $p$, so, these rays cut $\C$ in $v_p$ sectors. Let $S$
be one of these sectors, then $S$ is invariant under an
appropriate iterate of $f_c$, say $f_c^k$, where $k$ is a multiple
of the period $m$.

Now, every ray landing at $p=\pi(\h{p})$ lifts to a landing ray in
$L(\h{p})$. As in the dynamical plane, landing rays cut the leaf
$L(\h{p})$ also in $v_p$ sectors. We will check that when $p$ is
not in the dynamic root cycle, for each sector $\h{S}$ in $L$
there is an unbounded subset $\h{E}$ of the Julia set
$\mc{J}_{c}$. In fact, suffices to find a subset $\h{E}$ in
$\mc{J}_c\cap L$ invariant under the action of $\h{f}_c^k$. Since
$\h{f}_c^k$ is a similarity, the set $\h{E}$ would be unbounded.

To do that, let us construct a fundamental piece to the action of
$f_c^k$ in $\C$. Every sector $S$ contains a subset $E$ of the
Julia set. Let us take a point $b$ in $J(f_c)\cap S$, very close
to $p$, and such that there is a pair of rays $R_{b}$ and $R'_{b}$
landing at $b$, whose images $R_{f^k_c(b)}$ and $R'_{f^k_c(b)}$
belong to the wake $W_S$ determined by $R_b$ and $R'_b$. For
instance, $b$ can be a preimage of the dynamic root point, since
the set of such preimages is dense in the Julia set. Fix an
equipotential $E_r$ and join consecutive landing rays by arcs of
this equipotential. We obtain a region $P$ around $p$. The image
$f_c^k(P)$ is a region around $p$ and complactly contains $P$. The
annulus $A=\overline{P\setminus f_c^{k}(P)}$ is the fundamental
piece we are looking for, see Figure~\ref{fig.unbounded1}.

\begin{figure}[htbp]
\begin{center}
\input{unbounded1.pstex_t}
\caption{The annulus $A$ when $p$ is not in the dynamic root
cycle.} \label{fig.unbounded1}
\end{center}
\end{figure}

The Julia set intersects the annulus $A$ at the wake $W_S$ defined
by the rays $R_b$ and $R'_b$, thus for every $S$, we can enclose
the subset of the Julia set in $A\cap W_S$, in a simply connected
open set $V_S$ contained in $A\cap W_S$.

Now, $A$ lifts to an annulus $\h{A}$ in $L$, which by
construction, is a fundamental region for the action of
$\h{f}_c^k$. By iterating $\h{f}_c^k$ on $\h{V}_S$, the lifts of
the sets $V_S$, we obtain a set in $L$, similar to a pearl beds
string, which contains the subset of the Julia set $\h{E}$ in
$\mc{J}_c$ that we claim before. By construction, this pearl beds
string is unbounded and, there is one for each sector $S$. The
conclusion follows.

When $p$ is the dynamic root point $r_c$, each Fatou component
attached to $p$, lifts to another unbounded Fatou component in
$L(\h{p})$. In this case, let $S$ be a sector that contains a
Fatou component, say $F_S$, having $p$ in the boundary. Instead of
the point $b$ as above, we consider a pair of points $q$ and $q'$
on $\partial F_S$ and on opposite sides of $p$. There is two pairs
of landing rays, $\{R_q,I_q\}$ and $\{R_{q'},I_{q'}\}$ landing at
$q$ and $q'$, the names $R$ stand for external and $I$ for
internal rays. On the basin of infinity we follow the same
construction as in the case before, whereas in $F_S$ connect the
internal rays $I_q$ with $I'_q$ by a internal equipotential. So we
obtain again a puzzle piece $P$ around $p$, see Figure
\ref{unbounded2}. From now on, the argument above goes through
either for $S$ or sectors that do not contain Fatou components
attached to $p$.
\end{proof}

\begin{figure}[htbp]
\begin{center}
\input{unbounded2.pstex_t}
\caption{The annulus $A$ when $p$ belongs to the dynamic root
cycle.}
 \label{unbounded2}
\end{center}
\end{figure}

The following proposition gives another restriction that
combinatorics impose in the leaf structure of the Julia set.
However, it works in a more weak generality.


\subsection{Hyperbolics components}

As we pointed before, combinatorially, the Julia sets associated
to parameters within a hyperbolic component $H$ and the root of
$H$, are indistinguishable. Here, we present a proposition that
topologically ties the regular parts of parameters inside
hyperbolic components with the regular part of their center.

Although it was not explicitly stated the proof of next
proposition follows immediately from Lemma 11.1 in Lyubich and
Minsky's. We include the settings and the statement of that lemma
for reference. The interested reader can find the proof on
\cite{LM}.

Let $U$ and $V$ two open sets with $\bar{U}\subset V$ and let
$f:U\rightarrow V$ be an analytic branched covering. Let us remark
that when $U$ and $V$ are disks with the property $U\subset
\subset V$ the map $f$ is called \textit{polynomial-like} or
\textit{quadratic-like} if the degree of $f$ is $2$, let
$\mc{N}_f$ denote the set of backward orbits of $f$. In this
setting, iterations of the map $\h{f}$ on $\mc{N}_f$ may not be
defined, since $f$ is not defined on $V\setminus U$. For
$m=1,2,...$ let $\mc{N}_m\subset \mc{N}_f$ be the set of backward
orbits $\h{z}$ that can be iterated under $\h{f}$ \textit{at most}
$m$ times. So, we have inclusions $\mc{N}_m\subset \mc{N}_{m+1}$
for $m=1,2,...$.

The map $\h{f}^{-m}:\mc{N}_f \rightarrow \mc{N}_f$ is an
immersion, that maps $\mc{N}_f$ onto $\mc{N}^{m}$ for $m=1,2,...$.
So, by composing with the inclusions $\mc{N}^{m}\hookrightarrow
\mc{N}_f$ consider $\mc{N}_f$ as an extension of $\mc{N}^{m}$ and
let us denote these extensions by $\mc{N}^m$. Make
$\mc{N}_f=\mc{N}_0$ and identify any point $\h{z}\in \mc{N}^m$
with $\h{f}^{-1}(\h{z})$, so the map $\h{f}^{-1}$ induces the
following increasing sequence of sets
$$\mc{N}^0\hookrightarrow\mc{N}^1\hookrightarrow \mc{N}^2\hookrightarrow...$$
let $\mc{D}_f=\cup \mc{N}^m$, a set $W$ in $\mc{D}_f$ is said to
be open if $W\cap \mc{N}^m$ is open for every $m$. The set
$\mc{D}_f$ is called the \textit{direct limit} of the increasing
sequence above. The natural extension $\h{f}$ of $f$ in $\mc{N}_f$
induces a homeomorphism of $\mc{D}_f$ into itself. Now, we can
state the following Lemma:

\begin{lemma}[Lyubich and Minsky]\label{lem.11.1}
Assume that a branched covering $f:U\rightarrow V$ is the
restriction of a rational endomorphism $R:\bar{\C}\rightarrow
\bar{\C}$ such that $\C\setminus V$ is contained in the basin of
attraction of a finite attracting set $A$. Then
$\h{f}:\mc{D}_f\rightarrow \mc{D}_f$ is naturally conjugate to
$\h{R}:\mc{N}_R\setminus \h{A} \rightarrow \mc{N}_R \setminus
\h{A}$.
\end{lemma}

\begin{proposition}\label{attract.sup} The regular part of a
quadratic hyperbolic map is homeomorphic to the regular part of
its corresponding superattracting map.
\end{proposition}

\begin{proof} First, let us discuss parameters inside the Main Cardioid.

Let $f_{\epsilon}(z)=z^2+\epsilon$ a quadratic polynomial with
$\epsilon$ a parameter inside the Main Cardioid. Thus
$f_{\epsilon}$ has an attracting fixed point $a_{\epsilon}$. The
Fatou set consists of two open sets corresponding to the basins of
infinity $A(\infty)$ and $A(a_\epsilon)$. The Julia set
$J(f_{\epsilon})$ is a quasicircle, so that the conjugating map
$\phi:J(f_\epsilon)\rightarrow \mathbb{S}^1$ can be
quasiconformally extended to a neighborhood of $J(f_\epsilon)$.
Since $f_\epsilon$ is expanding on the Julia set, the map
$\phi\circ f_\epsilon \circ \phi^{-1}$ is an expanding circle map
of degree 2.

By a Theorem of Shub the map $\phi\circ f_\epsilon \circ
\phi^{-1}$ is topologically conjugate to $z^2$, that is, there is
a map $h:\mathbb{S}^1\rightarrow \mathbb{S}^1$ such that
$f_0=h\circ \phi\circ f_\epsilon \circ \phi^{-1} \circ h^{-1}$.
Also, $h$ admits an equivariant extension to a neighborhood of
$\mathbb{S}^1$. Actually, B\"ottcher's coordinate in the basin of
infinity extends $h$ to the whole basin of infinity. So we obtain
a conjugacy of $f_\epsilon$ to $f_0$ defined on a simply connected
neighborhood $U$ containing the basin of infinity and the Julia
set $J(f_\epsilon)$. We can choose $U$ small enough such that the
map $f_\epsilon :U\ra V$ is quadratic-like. This implies that the
map $f_\epsilon:U\rightarrow V$ is topologically equivalent to the
map $f_0:\phi(U)\rightarrow \phi(V)$. By construction,
$\C\setminus V$ is contained in the basin of attraction of
$a_\epsilon$.

By Lemma~\ref{lem.11.1}, the map
$\h{f}_\epsilon:\mc{D}_{f_\epsilon}\rightarrow\mc{D}_{f_\epsilon}$
is conjugate to $\h{f}_\epsilon:\mc{N}_{\epsilon}\setminus
\h{a}_\epsilon \rightarrow \mc{N}_{\epsilon}\setminus
\h{a}_\epsilon$, also the map $\h{f}_0:\mc{D}_{f_0}\rightarrow
\mc{D}_{f_0}$ is conjugate to $\h{f}_0:\mc{N}_0\setminus \h{0}
\rightarrow \mc{N}_{0}\setminus \h{0}$. But, the conjugacy $\phi$
from $f_\epsilon$ to $f_0$ lifts to a conjugacy from
$\h{f}_\epsilon:\mc{D}_{f_\epsilon}\rightarrow\mc{D}_{f_\epsilon}$
to $\h{f}_0:\mc{D}_{f_0}\rightarrow\mc{D}_{f_0}$. So,
$\mc{R}_\epsilon=\mc{N}_\epsilon \setminus
\{\h{\infty},\h{a}_\epsilon\}$ is homeomorphic to
$\mc{R}_0=\mc{N}_0 \setminus \{\h{\infty},\h{0}\}$.

It follows that $\mc{N}_\epsilon$ is homeomorphic to the double
cone over $\sol$. Let us remark that since the homeomorphism above
is a conjugacy, it sends the Julia set $\mc{J}_\epsilon$ onto
$\sol=\mc{J}_0$, so we can restrict such homeomorphism to the lift
of the basin of attraction of $a_\epsilon$, therefore
$\inver(f_\epsilon, A(a_\epsilon))\cup J(f_\epsilon)$ is
homeomorphic to $\cone$.

Let $f_c(z)=z^2+c$ be a quadratic polynomial with $c$ in a
hyperbolic component $H$, with attracting cycle
$P=\{p_1,...,p_n\}$ of period $n$. Let $U_1,U_2,...,U_n$ be the
Fatou components of the basin of attraction of $P$.

The regular part $\mc{R}_c$ can be decomposed in several parts, by
cutting along the Julia set $\mc{J}_c$ which are:

\begin{itemize}

\item The Julia set $\mc{J}_c$.

\item The lift of the basin at infinity $\pi^{-1}(A(\infty))$ in
$\mc{R}_c$.

This set is homeomorphic to $\sol \times (0,1)$ by means of the
lift of B\"ottcher's coordinate.

\item Fatou components of finite branching.

This set is homeomorphic to a countable union of sets
$\{\mc{V}_n\}$, where each $\mc{V}_n$ is homeomorphic to
$\mathbb{D}\times \cantor$. Each point $\h{z}\in \mc{V}_n$ has at
most finitely many coordinates in the basin of attraction of the
critical cycle $\cup U_j$. Also, each component in $\mc{V}_n$
projects onto some $U_i$ for $i$ fixed.

\item The invariant lift $\h{U}$ of the basin of attraction of
$P$.

Let $\h{U_i}$ be the of points $\h{z}\in\h{U}$ such that
$\pi(\h{z})\in U_i$, with the lift of K\"oning's coordinate on
$\h{U}_i$, $\h{f}^n_c$ has the form of $z\mapsto \lambda z$, where
$\lambda$ is the multiplier of the cycle $P$, so $\h{f}^n_c$ in
$\h{U}_i$ is topologically equivalent to $\h{f}_\lambda$ in
$\pi^{-1}(A(a_{\lambda}))$. By the discussion above, $\h{U}_i$ is
homeomorphic to $\sol\times (0,1)$.

\end{itemize}

Let $c_0=H(0)$ be the center of $H$. Now, the regular part
$\mc{R}_{c_0}$ has the same decomposition as $\mc{R}_c$, the
decomposition is such that the corresponding components are
homeomorphic. These homeomorphisms glue together to a
homeomorphism from $\mc{R}_c$ to $\mc{R}_{c_0}$. \end{proof}

We call the decomposition of $\mc{R}_c$ above, the
\textit{laminated decomposition} of the regular part associated to
the hyperbolic parameter $c$. Tomoki Kawahira independently proved
Proposition~\ref{attract.sup} in the more general setting of
hyperbolic rational maps and in the quasiconformal level. That is,
hyperbolic affine laminations are stable in Lyubich-Minsky
setting. See \cite{Tom2}. Let $H$ be a hyperbolic component, and
$c_0=H(0)$ be the center of $H$. For any hyperbolic parameter $c$
in the boundary of $H$, the path from $c_0$ induces a
transformation $h_c$ from $\mc{R}_{c_0}$ to $\mc{R}_c$. If
correspondingly $c_1$ denotes the root of $H$, then $f_{c_1}$ is a
parabolic quadratic polynomial. Let $\mc{L}$ be the regular part
of $\mc{R}_{c_0}$ with the leaves containing the dynamic root
cycle removed. Analogously, let $\mc{L}'$ be set obtained by
removing from $\mc{R}_{c_1}$ the periodic leaves associated to
Fatou's coordinate. Then, another result of Kawahira, see
\cite{Tom}, states that the map $h_{c_1}=\lim h_c$, as $c$ tends
to $c_1$ in $H$, is a laminar homeomorphism between $\mc{L}$ and
$\mc{L}'$, and moreover, the map $h_{c_1}$ semi-conjugates
$\h{f}_{c_0}|_{\mc{L}}$ to $\h{f}_{c_1}|_{\mc{L}'}$.

%\begin{proposition}[Kawahira] The map $h_c$ is a semi-conjugacy
%from $\mc{R}_{c_0}\setminus \h{P}$ to $\mc{R}_c$, such that the
%restriction of $h_c$ to $\mc{R}_{c_0}\setminus \{$leaves
%containing the cycle $\h{P}\}$ is a laminar homeomorphism into
%$\mc{R}_{c}\setminus \{$leaves containing the parabolic cycle of
%$c\}$.
%\end{proposition}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ordenado"
%%% End:

